SME: ReRAM-based Sparse-Multiplication-Engine to Squeeze-Out Bit Sparsity of Neural Network

Resistive Random-Access-Memory (ReRAM) crossbar is a promising technique for deep neural network (DNN) accelerators, thanks to its in-memory and in-situ analog computing abilities for Vector-Matrix Multiplication-and-Accumulations (VMMs). However, it is challenging for crossbar architecture to exploit the sparsity in the DNN. It inevitably causes complex and costly control to exploit fine-grained sparsity due to the limitation of tightly-coupled crossbar structure. As the countermeasure, we developed a novel ReRAM-based DNN accelerator, named Sparse-Multiplication-Engine (SME), based on a hardware and software co-design framework. First, we orchestrate the bit-sparse pattern to increase the density of bit-sparsity based on existing quantization methods. Second, we propose a novel weigh mapping mechanism to slice the bits of a weight across the crossbars and splice the activation results in peripheral circuits. This mechanism can decouple the tightly-coupled crossbar structure and cumulate the sparsity in the crossbar. Finally, a superior squeeze-out scheme empties the crossbars mapped with highly-sparse non-zeros from the previous two steps. We design the SME architecture and discuss its use for other quantization methods and different ReRAM cell technologies. Compared with prior state-of-the-art designs, the SME shrinks the use of crossbars up to 8.7x and 2.1x using Resent-50 and MobileNet-v2, respectively, with less than 0.3% accuracy drop on ImageNet.

==> Sec3-SME-algorithm_original.tex <==

\section{SME Algorithm}
\subsection{SME Algorithm Overview and Key Innovations}

\begin{figure*}[thb]
\setlength{\abovecaptionskip}{3pt}
\centering
\includegraphics[width=1.0\linewidth]{image/algorithm-overview-v2.pdf}
% \includegraphics[scale=0.3]{image/distribution-new-crop.pdf}
\caption{The overview of proposed algorithm framework is composed of three parts, and six steps are needed to finish the whole process. We first quantize weight matrix to present them in binary with bit-sparse pattern. Then, the weights are splitted onto several bit matrices by our mapping scheme. After that, we squeeze out the inter- matrix sparsity by row squeezing while eliminating the value bias generated on weights.}
% \caption{The overview of the proposed algorithm framework, which consists of (1), (2), and (3) in the figure. First, we quantize the weights by exponent-based quantization (Step 1) produces massive and regular sparsity after binary encoding (Step 2). Then, the quantized weight matrix is split into eight bit-matrices, and different bits of weight locates the same position in the bit matrix (Step 3). Next, we squeeze the bit matrices along the bit-with to reduce the crossbar resources occupied by these sparse but significant bits, which can also be reserved. That is, Step 4 starts from the bit matrix storing MSB, among which non-empty rows are placed in the same position as the back bit matrix in proper order, and the squeezed row of the bit matrix stores LSB is discarded. Finally, we further flip the bits to produce sparsity (Step 5) and through the compensation mechanism to reduce the changes in weight caused by flip-bit (Step 6). Step 5 and Step 6 start from the bit matrix storing MSB, and are executed iteratively on the back bit matrix. The column on the right shows that the above execution process is converted into 3D for operation.} 
\label{fig:algorithm-framework}
\end{figure*}

Our SME mapping algorithm includes three parts: quantization, inter-crossbar mapping and squeezing. The quantization method should bring us structured bit-level sparsity, and the mapping scheme should enable us to treat the contents in different bits separately to exploit the different sparsity rates. In addition, noticing the extreme sparsity in the most significant bits, we propose the squeeze scheme to decouple their position and calculation result without introducing extra indices.

% We propose a mapping algorithm framework to exploit the bit-level sparsity of weight matrix, also known as the ``0'' bits in the binary representation. The key idea is to reorganize the bits of the weight matrix with the architecture support to generate the structured bit-level sparsity that is used to be expensive and almost impossible to use in conventional architecture. 

% According to Fig.~\ref{fig:distribution}, we can see that there are bit-level sparsity in 

% The mapping algorithm framework contains four steps to map the weight bits on to SLC ReRAM-crossbars, as depicted in Fig.~\ref{fig:algorithm-framework}:
The overview of our SME algorithm is depicted in Fig.~\ref{fig:algorithm-framework}:
\begin{itemize}
\item
In Step~\hquan{1} and \hquan{2}, we quantize and encode the weights based on an extension of power-of-two quantization method~\cite{li2019additive}, which round the weight to the third bit from its most significant bit. \emph{This method limit the maximum number of `1's that may appear in the binary codework with minimal relative error.}
% In Step~\hquan{1} and \hquan{2}, we quantize the weights based on an extension of power-of-two quantization method~\cite{li2019additive}, and then encode the quantized weights into a binary codeword. In the resulting $N$-bit codeword, an `1' in $i$ bit represents a value $2^{-i}$. \emph{The innovation is that we quantize and encode the weight so that `1' will only appear in $S$ successive positions~(e.g., $S \leq 3$ for $N=8$), and the positions can be decided according to the magnitude of the weight.} After mapping to the SLC ReRAM crossbar, we can observe a regular sparse pattern: the zero bits are accumulated in the head and/or tail of the codeword. The proposed quantization method can preserve the model accuracy and avoid incurring any retraining steps, similar to INT8~\cite{jacob2018quantization}, but is more hardware-friendly.

\item
In step \hquan{3}, we map the same bit of every weights into the same crossbar. Different bits from a weight is separated in the same position of every crossbar under this mapping scheme, namely inter-crossbar mapping. Therefore, a $W\times H$ weight matrix quantized with $W$ bits will be mapped into $N$ bit matrices (denote as BM) of size $H\times W$.
% According to Fig.~\ref{fig:distribution}, we found that the bit-level sparsity differs greatly over different bits. Mapping different bit in the same crossbar makes it impossible to implement customized acceleration effort for each bit. Therefore, we map a $W\times H$ weight matrix quantized with $W$ bits into $N$ bit matrices (denote as BM) of size $H\times W$, shown as step~\hquan{3}.
% Similar to~\cite{yang2019sparse,chu2019pimprune}, it is difficult to exploit sparsity effectively and skip these irregular zero bits due to the tightly coupled crossbar structure. Step~\hquan{3} of our mapping framework, however, splits the weight matrix bit-wisely into $N$ bit matrices (denote as BM) of size $H\times W$. \emph{This innovative mapping method can accumulate the sparsity in the same crossbar}. For example, the crossbar mapped with BM$_1$~(head bits) and BM$_8$~(tail bits) are extremely sparse and thus can be easily exploit later. Fig.~\ref{fig:algorithm-framework} also shows a 3D view of the bit matrices organization.

\item
In Step~\hquan{4}, we squeeze the rows which are not empty in BM$_1$ to the next BM, to empty BM$_1$. A corresponding operation on the input of these rows is also performed.
%squeeze the rows containing non-zero bits~(namely non-empty rows) out of BM$_1$ and replace the corresponding rows in BM$_2$. The rows of BM$_2$ losing their positions are subsequently squeezed to BM$_3$. This procedure continues until the rows of BM$_N$ are dropped out. This squeeze-out method can empty the BM$_1$ and/or BM$_2$. \emph{This innovative squeeze-out method makes full use of the derived sparse pattern to reduce the crossbars storing the extremely sparse MSBs at the lowest expense~(i.e., accuracy drop) of dropping out the LSBs}. The squeeze-out of weight bits incurs very limited hardware overhead for matching of input~(detailed later). 

% \item
% Step~\hquan{5} judiciously flips $1\rightarrow 0$ in the bit matrices to minimize the maximal number of `1's in a crossbar-column, targeting at increasing the number of rows of crossbar cells for concurrent execution of MACs.Subsequently, we compensate the change of weight bits by flipping $0\rightarrow 1$ in the less significant bit matrices in Step~\hquan{6}. % \emph{This iterative procedure can easily converge with minimum change of weight values because bits in the bit matrix belong to different weights and are thus independent. Otherwise, one $1\rightarrow 0$ flipping may incur more $0\rightarrow 1$ flipping in the same bit matrix derived by conventional mapping.} Moreover, the bonus of the flip operation is the emergence of empty columns that can be further squeezed-out with limited hardware overhead of the alignment of results~(detailed later). 
\end{itemize}
% Given a pre-trained DNN model, we first apply an existing quantization method ~\cite{li2019additive}, which can preserve the model accuracy without incurring any retraining steps. By applying the proposed Encoding Scheme, the weight matrix reveals a special bit-sparse pattern. Then, we use the Bit-Wise inter-crossbar Mapping method to regroup and transform the weight matrices to bit-matrix. This step cumulates the zero bits in the whole crossbar, and consequently we can Squeeze-out the non-zero bits with ignorable change the weight value. The algorithm framework can fully exploit the bit-level sparsity for our purpose without actually pruning any weights.
\subsection{Sparse Pattern and Mapping Scheme}
\label{sec:mapping}

\begin{figure}[htbp]
\centering
\includegraphics[scale=0.14]{image/comparsion_INT8_v2.pdf}
\caption{Comparison of conventional INT8 quantization (a) and logarithmic quantization (b) for deploying model onto SLC-based crossbars.}
% \caption{Comparison of our method and conventional method for deploying the model to crossbars. (a) The conventional method leads to scattered distribution of sparsity on crossbar. (b) Our quantization generates massive and structural sparsity on the crossbar. (c) The massive sparsity is decoupled with crossbar and can be used to save crossbar resources, which benefits from the combination of our encoding and mapping.}
% \caption{Our quantization \& inter-crossbar mapping scheme vs. conventional quantization \& intra-crossbar mapping. (a) Deploy the quantized weights by INT8 to the crossbar with conventional mapping method, resulting in scattered distribution of sparsity on crossbar. (b) Due to our quantization, there is massive and regular sparsity on the crossbar, but the sparsity is tightly coupled with the crossbar, which leads to utilizing to save resources difficultly. (c) The massive sparsity is decoupled with crossbar and can be used to save crossbar resources, which benefits from the combination of our encoding and mapping.}
\label{fig:comparsion-int8}
\end{figure}

% Following our motivation, the quantization should have the following properties: the result should be encoded in binary; the `1' bits in the result should be structured but as few as possible; the accuracy loss should be negligible. 

% Therefore, we carry out the quantization scheme that every weight is encoded into $N$ bits and is rounded to the $S$-th bit from its most significant bit. The encoded binary representation $b_{1:S}$ of a weight $w$ can be expressed as
% \begin{align*}
%     & \quad b_{1:S} = \mathop{\mathrm{argmin}}\limits_{b_{1:S}} \left| w - \sum\limits_{i=1}^S b_i 2^{-i} \right|\\
%    \mathrm{s.t.} & \quad b_k= \begin{cases}
%         0\ \mathrm{or}\ 1, & k = msb, msb+1, \cdots, msb+S-1\\
%         0, & \mathrm{otherwise}
%     \end{cases}
% \end{align*}
% Here $msb$ is the most significant bit of $w$. Sometimes the range of weights in a layer doesn't match the range of quantization, whose maximum quantized value is $1-2^{-S}$. A shift operation will be carried out to the weights $W_l$ of the $l$-th layer. 
%     \begin{align*}
%         w' &= w \times 2^m\\
%         m &= \mathop{\max}_k \left\{2^k\times \max(\mathrm{abs}(W_l)) \leq 1 - 2^S\right\}
%     \end{align*}
% The object of weight quantization we needed is to identify a binary representation using as few `1's as possible, instead of simply reducing the bit-width in prior works, e.g., INT8~\cite{jacob2018quantization}. By combining the weight encoding format deployed on the crossbar, the weight matrix reveals a special bit-sparse pattern. In the resulting $N$-bit codeword, an `1' in $i$ bit represents a value $2^{-i}$. The innovation is that we quantize and encode the weight thus `1' will only appear in $S$ successive positions~(e.g., $S \leq 3$ for $N=8$), and the positions can be decided w.r.t the magnitude of the weight. This restricts the relative quantization error well~(1/8 of value with $S=3$) and also provides sparsity that is convenience for squeeze-out (in~\ref{para: squeeze-out}). Therefore, we introduce the novel quantization~\cite{li2019additive} with the sparse pattern, as shown in~\ref{fig:comparsion-int8} (a) and (b), APT quantization with the sparse pattern generates greater amount of and more regular sparsity on the crossbar with conventional mapping method, compared with INT8. 
% Also, to restore the original value, INT8 needs to multiply with a floating number ($1/255$ in the example) while APT quantization only need to multiply with a power-of-two value, which can be implemented with hardware-friendly shift operation. Both differences make our method work better. \par
% As shown in Fig.~\ref{fig:comparsion-int8} (a) and (b), deploy the quantized weights by INT8 to the crossbar with conventional mapping method, resulting in the scattered distribution of sparsity on crossbar. In contrast, there is massive and regular sparsity on the crossbar quantized by logarithmic quantization.
% Even the more bit-level sparsity, however, cannot be exploited to improve the crossbar performance. \par


Due to the tightly coupled crossbar structure, however, even the more and regular bit-level sparsity, it is challenging to exploit sparsity to improve the crossbar performance efficiently.
To solve the problem, we introduce the \textbf{bit-split and inter-crossbar} mapping scheme that stores the same bits from different weights into the same crossbar.
As shown in Fig.~\ref{fig:algorithm-framework}, a weight matrix with size $W\times H$ quantized with $C$ bits is split into $C$ bit-matrices with same size $W\times H$, and each bit matrix is deployed to several crossbars from one group. Each bit of a quantized weight locates in its corresponding bit crossbar (bit-split), and different bits of the weight locate in the same position of all bit crossbars (inter-crossbar). This is equivalent to mapping to a 3D structure, which is called ``3D-Cube''.

Our sparse pattern and mapping scheme is equivalent to accumulating the dot product of the iteration bit with the shift of constant (in Equation~\ref{con:equ1}), and requires same shifter and adder as the requirement in conventional mapping method, but only modify the peripheral circuit (refer to Section~\ref{sec:modules}).
\begin{equation}
\setlength\abovedisplayskip{3pt}%shrink space
\setlength\belowdisplayskip{3pt}
weight = \sum_{i=1}^{bitwidth} b_i\cdot 2^{-i}, \quad b_i\in\{0,1\}
\label{con:equ1}
\end{equation}
wherein $b_i$ indicates the $i$-th bit in binary codeword, which represents a value $2^{-i}$. $\sum_{i=1}^{bitwidth}$ represents accumulate all the values of `1' in the binary codeword.


% The motivation of this mapping method is that the numbers of `1's on different bits vary greatly (Fig.~\ref{fig:distribution}). Different bits have different sparsity, such as the bits in the middle is very dense in `1's while the most significant bits are at the opposite extreme, very sparse. By distributing the bits from different digits into different crossbars, these crossbars have their sparsity and importance, which provides more high operational flexibility and possibility through loosing coupling, greatly improved the efficiency to apply operation for each bit.

% Besides, Fig.~\ref{fig:distribution} also shows the comparison of the bit distribution between INT8 and our quantization.The target of our quantization scheme is to find a binary representation for the weights with minimum numbers of `1's to increase sparsity while retaining their values. Our quantization method is designed on the basis of APoT~\cite{li2019additive}, which quantizes weights into sums of several power-of-two terms. Combining with our target, we perform the following quantization scheme.



% To minize the number of `1's as well as retaining the original value as much as possible, we first find the approximation of weights with several \textbf{effective digits(bits)} in binary and the effective digits(bits) represents the continuous `1' in the binary. In addition, since all the weights in a convolution layer share the same \textbf{presenting bit} positions, we choose the most significant presenting bit as the MSB of the largest weight in the whole layer to make full use of the bit width. In the following discussion, the most significant presenting bit is set to be $2^{-1}$ to ease expression and changing it only requires a shifter, which only have negligible overhead. Any bit that is out of the range of presenting bits will be discarded.

% For example, we want to quantize number 0.361 with 8 presenting bits and 3 effective digits. Its binary presentation is $0.01011100..._{2}$. Quantizing the number with 3 effective digits gives us $0.375 = 0.0\mathbf{110}0000_2$ and the bits saved in crossbars will be 01100000.
% Moreover, although $2^{-8} + 2^{-10}$ have 3 effective digits, but $2^{-10}$ is out of the range of presenting bits and the number will be quantized to $2^{-8}$.



% After quantizing the weights, the conventional bit-wise mapping method maps the bits of a quantized weight onto adjacent ReRAM-crossbar cells~\cite{shafiee2016isaac,chi2016prime,chou2019cascade,yao2020fully}, namely intra-crossbar mapping. The crossbar with this mapping method exhibits column-wise sparsity. For example, a column of crossbar mapped from the MSBs is very likely to be empty, but its adjacent columns may not. Such bit-level~(i.e., column) sparsity, however, cannot be exploited to reduce the crossbar footprint. 

% To solve the problem, we introduce the \textbf{bit-wise and inter-crossbar} mapping scheme that stores the bits from different digits into different crossbars.

% The motivation of this mapping method is that the numbers of `1's on different bits vary greatly(Fig~\ref{fig:distribution}). The bits in the middle is very dense in `1's while the most signicant bits are at the opposite extreme, very sparse. By distributing the bits from different digits into different crossbars, these crossbars have their own sparsity and importance. Therefore, we can define different prune ratio for each bit crossbar. For dense but less significant bit crossbars, we can define a large prune ratio while we can define a low prune ratio for sparse and significant ones, or even do not prune them.

% A weight matrix with size $W\times H$ quantized with $C$ bits is split into $C$ bit-matrices with same size $W\times H$, and each bit matrix is deployed to several crossbars from one group. Each bit of a quantized number locates in its corresponding bit crossbar (bit-split), and different bits of weight locates the same position in the bit crossbar (inter-crossbar). This is equivalent to mapping to a 3D structure, which is called ``3D-Cube''.

% Our encoding and mapping scheme is equivalent to accumulating the dot product of the iteration bit with the shift of constant (in Equation \ref{con:equ1}), and requires same shifter and adder as the requirement in conventional bit-wise mapping method, but only modify the peripheral circuit.
% \begin{equation}
% \setlength\abovedisplayskip{3pt}%shrink space
% \setlength\belowdisplayskip{3pt}
% psum = I \times \sum_{i=1}^{bitwidth} b_i\cdot 2^{-i}, where~b_i\in\{0,1\}
% \label{con:equ1}
% \end{equation}

% Using our mapping scheme, a weight matrix with size $W\times H$ quantized with $C$ bits will be mapped into a three-dimension crossbar with size $W\times H\times C$. Each bit of a quantized number locates in its corresponding bit crossbar (bit-split) and all the bits at the same position of bit crossbars form the corresponding weight (inter-crossbar).


% \subsection{Encoding scheme}
% \label{sec:encoding}
% We quantize the weights by additive exponent-based quantization method~(e.g., APoT~\cite{li2019additive}). Their principle is to approximate the original weight using the sum of power-of-two terms with the decreasing exponents. Their purpose is for a good tradeoff between the range and granularity of quantized numbers. For example, the number $0.78$ is quantized to $0.75 = 2^{-1}+2^{-2}$. Based on previous study, this quantization method can preserve the accuracy of various large CNN models with $4$ bits in the Imagenet dataset. The codeword of the resulting quantized number is a set of binary codes, representing the sign bit, and the set of exponents. %AUSN~\cite{fangxin2020ausn} apply the above quantization method to both feature maps~(activation) and weight, so that the accelerator can substitute the costly multiplication with shift operation.

% %the encoding scheme, as shown in Algorithm~\ref{alg:coding-algorithm}, . And the codeword consists of the bits represented by the exponent. Then, according to the parameter s, which represents the maximum number (e.g., $s=3$) of `1's exists in codeword,

% In this work, we investigate the above quantization method in crossbar structure. 


% As a result, we find the bit-level sparsity generated by encoding the weight matrix quantized by the exponent-based quantization method is more regular against other quantization methods. Therefore, we extract the sparsity exists in the codeword of quantized weights into a special sparse pattern, which 
% the `1's appear in the codeword must be continuous and less than $s$, making the distribution of `0's is regular.


% For example, suppose the $s=3$, the quantized number $0.3671875$ by INT8 encoded as ``$01011110$'' can be quantized by exponent-based quantization method, which is encoded as ``$01100000$'' of $0.375$. It can be seen that the bit-level sparsity produced by encoding the original value is scattered and unstructured, which is difficult to be exploited. However, with the exponent-based quantization method, the number of `1's is 2, which is less than $s=3$ and the `0's in the codeword is more regular and massive. And the quantized value is also closest to the original value.

% For a fair comparison, we quantize weights from 32-bit to 8-bit. However, this quantization method is also applicable to other bit-width and still keeps the pattern.
% % consecutive adjacent exponents. Consequently, most of these encoded bits stored in cell of crossbar exist $s$ `1's and must be adjacent, making 0s aggregated (as shown in Algorithm~\ref{alg:coding-algorithm}). 
% % We analyze the quantization method~\cite{li2019additive, fangxin2020ausn} to identify the form of exponents (of power-of-two) in different bit-width and make two observations. First, the binary representation of quantized weights naturally matches SLC-based crossbar since the weights are quantized to the form of exponents. As a result, lower overhead will be present in the binary transformation and can be easily mapped to crossbar. Second, there is the particular sparsity pattern among the quantized weights, which is the weights are represented by the superposition of $s$ consecutive adjacent exponents. Consequently, most of these encoded bits stored in cell of crossbar exist $s$ `1's and must be adjacent, making 0s aggregated (as shown in Algorithm~\ref{alg:coding-algorithm}).

% The encoding with the sparse pattern makes it possible for further sparsity utilization without accuracy loss.


% %
% %\begin{algorithm}[hb]
% %	\setlength\abovedisplayskip{0pt}%shrink space
% %	\setlength\belowdisplayskip{0pt}
% %	\caption{SLC-based Encoding with Sparse Pattern}
% %	\label{alg:coding-algorithm}
	
% %	\textbf{Input}: {Original weight $w$ % Weight $w$ with bit-width N, maximum number of superposition (`1') $n$, power basis for each superposition $\mathcal B_i$}\\ %, i=1,\cdots, n$
% %	}\\
% %	\textbf{Parameter}: Presenting bit-width $N$, significant digit $s$\\
% %	\textbf{Output}:  \hspace{-1mm}
% %	{The quantized number $w_q$ and its encoding $E_w$}
	
% %	\begin{algorithmic}[1] %[1] enables line numbers
% 		% \STATE Let $rem\leftarrow w$, current superposition number $tier\leftarrow0$\;
% 		% \FOR{$k < N$}
% 		% \STATE        $E_w[k+1] = 0$
% 		% \ENDFOR
% %		\STATE Initialize $E_w = 00\cdots0$, length = $N$. $rem = w$, $w_q = 0$.
% %		\STATE $MSB$ = $\lfloor\; \log_2 w \;\rfloor$

% %		\FOR{$i$ in range($s$)}
% %		\IF{ $|MSB - i| < N$ and $2 ^ {MSB - i} < rem$ }
% %		    \STATE $rem = rem - 2 ^ {MSB - i}$
% %		    \STATE $w_q = w_q + 2 ^ {MSB - i}$
% %		    \STATE $E_w[|MSB - i|] = 1$
% %		\ENDIF
% %		\ENDFOR
		
% %		\STATE return $w_q$, $E_w$.
% 		% \WHILE{$rem>0$ {\rm and} $tier\leq n$}
% 		% \STATE  $w_q[tier] = \mathop{\rm argmax} \limits_p \mathcal \{B_{tier}[p] \leq rem\}$
% 		%$\max\{p|\mathcal B_{tier}[p] \leq rem\}$\;
% 		% \STATE        $rem = rem/ w_q[tier]$ -1 \;
		
% 		% \STATE        $tier$ += 1 \;
% 		% \ENDWHILE
% 		% \STATE        $w_p = abs( log_2 (w_q) )$
% 		% \STATE \textbf{return} $w_q=\mathop{{\rm 
% 		% 		Join}}\limits_{0\leq i\leq n} w_q[\,i\,]$\; $E_w=\mathop{{\rm 
% 		% 		Flip}}\limits_{0\leq i\leq n} E_w[w_p[\,i\,]]$
		
% %	\end{algorithmic}
% %\end{algorithm}
% %




% \subsection{Mapping}
% \label{sec:mapping}


% We statistically analyze the distribution of non-zero bits among all the 8-bit weights using the above encoding scheme, as shown in Fig.\ref{fig:distribution}. We observe 1) large amount of non-zero bits clustered in the middle bits, and 2) large amount of redundant zero-bits around Most-Significant-Bit~(MSB) and Least-Significant-Bit~(LSB). Such an observation conforms to the weight value distribution~(see the left-up small figures) and most existing quantization schemes (e.g. INT8~\cite{jacob2018quantization}). 

% % (Fig. 3: APOT-based encoding scheme vs. INT8-based encoding)

% %Meanwhile, effective mapping needs to start from the `1' among the bit-width involved to be calculated. All of the above enable us to create a bit-level splitting of existing dense DNN models.

% The conventional bit-wise mapping method splits a weight~(e.g., 8-bit) and maps these split bits into adjacent ReRAM-crossbar cells~\cite{shafiee2016isaac,chi2016prime,chou2019cascade,yao2020fully}, namely intra-crossbar mapping. The crossbar with this mapping method exhibits column-wise sparsity. For example, a column of crossbar mapped by the MSBs contains no 1-bit cell. Such bit-level~(i.e., column) sparsity, however, cannot be exploited to reduce the crossbar footprint. 

% We design a bit-wise and inter-crossbar mapping that can significantly reduce the nubmer of crossbars. The weight matrix of a convolution layer is mapped into a three-dimension structure. Two of the dimensions are same as the size of the weight matrix and indicates the location of the corresponding weight. The third dimension are used to partition each bit of the encoded weight and its length is the bit-width of encoding. After that, we map a $W\times H$ weight matrix encoded with $C$ bits into a $W\times H\times C$ 3-dimension crossbar and each cell is a single-level cell that stores either 0 or 1.
% % We design a bit-level splitting Mapping with significantly reduced redundant crossbar space. As a result, the implementation of DNN models mapping in the three-dimensional partitioning and mapping bits of weights matrix into relative locations (i.e., the location in the weight matrix) in the third dimensional represents the bit-width .

% Our mappings are equivalent to accumulating the dot product of the iteration bit with the shift of constant (in Equation \ref{con:equ1}), and requires same shifter and adder as the requirement in the conventional two-dimensional case , but only modify the peripheral circuit. Besides, our mapping strategy based on a universal occupancy weights matrix are especially useful for aggregating sparsity because of the bit distribution that DNN models generate. 
% \begin{equation}
% \setlength\abovedisplayskip{3pt}%shrink space
% \setlength\belowdisplayskip{3pt}
% psum = I \times \sum_{i=1}^{bitwidth} b_i\cdot 2^{-i}, where~b_i\in\{0,1\}
% \label{con:equ1}
% \end{equation}


\begin{figure}[ht!]
\centering
\includegraphics[scale=0.6]{image/row-Fig.pdf}
\caption{ An example about non-empty row statistics of the bit matrix storing MSB in each layer of the ResNet-18.}
\label{fig:row-statistic}
\end{figure}
\subsection{Bit-wise Squeeze-out}
\label{para: squeeze-out}
The bit-wise squeeze-out method is inspired under the following observations. The first few bit matrices are so sparse that they cannot even fill out a single crossbar. According to our quantizing scheme with the bit-sparse pattern, `1's will only appear in successive positions, which means that for the weights whose first few bits are `1', their last few bits must be `0'. We can have an empty bit matrix saving the MSB by squeezing-out these bits without changing the actual quantized weight. 

% The bit-wise squeeze-out method is inspired under the following observations. The proposed quantization results in a regular sparse pattern, e.g., $s$ `1' bits appear continuously with $s\leq 3$ in a 8-bit codeword. As shown in Fig.~\ref{fig:algorithm-framework} (2), if the first three most significant bits contains `1', then last three least significant bits must be `0'. Thus, we can safely squeeze-out at most three bit towards the LSB and drop out three `0' bits without changing the actual quantized weight. 

Since all the cells in the same crossbar-row share the same input, we decide to squeeze the whole row in the bit matrix once at a time for minimizing the overhead. Fortunately, our quantization with bit-sparse pattern and mapping scheme make sure that the first few most-significant bit matrices are highly sparse. A statistical analysis on the number/ratio of non-empty rows in the most significant bit matrix~(see  Fig.~\ref{fig:row-statistic}) shows that only 5\% to 10\% non-empty rows need to squeeze out in average. This evidence justifies the effectiveness of the squeeze-out method. %there are few non-empty rows in the MSB or the second-order bit matrix, which means the first few bit matrices are very sparse. To further reduce the crossbar resources occupied by these sparse but important bits while reserve them, we propose the squeeze-out strategy along bit-width based on above methods (Encoding and Mapping).

% After our mapping, each bit matrix stores the same bit. The same position in each bit matrix represents the different parts of the weight, and the order of bit represents the importance of the part in weight. By combining the our quantization method, we find the character in the bit matrices. If there are `1's in the first few matrices, then the same positions in the last few bit matrices always be `0', means large weights can tolerate LSBs variation. In the last bit matrix (represent the LSB), the bits on the locations will be squeezed and resulting in overflow, which will be drop out. It is worth noting that most of these squeezed positions in the higher significant bit matrix are `1', so the overflow part is mostly `0', which will not affect the accuracy of the model.

\begin{comment}
Suppose that the quantized weight matrix is $w_{W\times H}$ which mapped into a $W\times H\times C$ matrix $M$ consists of $C$ bit matrices:
    \begin{equation}
        w[i,j] = \sum\limits_{k=1}^C 2^{-k}M[i,j,k] = \sum\limits_{k=1}^C 2^{-k}BM_k[i,j]
    \end{equation} 
    
After squeeze out one bit along the bit-width direction, the squeezed matrix $M_{sq}$ has size $W\times H\times (C-1)$ and 
    \begin{equation}
         M_{sq}[i,j,k]= \begin{cases}
            0, & k=1\\
            M[i,j,k-1] & \sum\limits_{p=0}^W M[p,j,1] > 0, k>1\\
            M[i,j,k] & \sum\limits_{p=0}^W M[p,j,1] = 0\\
        \end{cases}
    \end{equation}
We got the squeezed matrix that the first layer the bit-width direction is all 0, which can be removed. We reserve its index for easier understanding.

Then, the weight matrix after squeezing $w_{sq}$ can be represented as
    \begin{equation}
        w_{sq}[i,j] = \sum\limits_{k=\mathbf{2}}^C 2^{-k}M[i,j,k]
    \end{equation}
    
Comparing with the equation for $M_{sq}$, we can see that the value from rows that is empty in the BM$_1$, the value remains the same. On the other hand, those rows who have content in the BM$_1$ dropped their content in BM$_8$ stores LSB and their value is also halved.
\end{comment}
% \begin{figure}[htbp]
% \centering
% \includegraphics[scale=0.2]{image/squeeze.pdf}
% \caption{An example of squeeze-out strategy.}
% \label{fig:squeeze}
% \end{figure}

% \begin{equation*}
% \begin{WithArrows}
% s.t.\quad O_1' &= O_1,
% b_{1,k}\in\{0,1\}\\
% O_1&= I_1\times W_1 + I_2 \times W_2,\quad W_1 = \sum_{k=1}^{bitwidth} b_{1,k}\cdot 2^{-k} \Arrow[jump=2]{squeeze\\first row} \\
% O_1' &= I_1'\times W_1' + I_2 \times W_2\\
% W_1' &= \sum_{k=1}^{bitwidth} b_{1,k}\cdot 2^{-(k+1)} \Longleftrightarrow W_1 >> 1\\
% I_1' \times  W_1' &\Longleftrightarrow I_1' \times  (W_1 >> 1)\\
% \rightarrow I_1' &= I_1 << 1 (I_1\times 2)

% % \Arrow[jump=1]{j=i-1, flip} \\
% % BM_{k}(P) & = M[P_x,P_y,{j}]  = 0
% \end{WithArrows}
% \end{equation*}

Aftre squeezing-out by one bit, the non-empty contents in BM$_i$ are moved to BM$_{i+1}$ and the contents in the last bit matrix is abandoned. According to Equation~\ref{con:equ1}, the value in that row is approximately halved with 1-bit squeezed. To ensure the invariance of the calculation results, we propose a scheme to double the input~(refer to Step \hquan{4} in Fig.~\ref{fig:algorithm-framework}). Note that we can even perform this step iteratively to squeeze-out multiple bits. The number of iteration is called the degree of squeeze-out. % The squeeze-out degree increases by 1 with squeezing 1-bit along the direction of bit-width. 
In this paper, we use the same style of input as in ISAAC~\cite{shafiee2016isaac}. The input is converted into bit-serial voltage and act on the crossbar for calculation. The number of cycles required is equal to the bit-width of the input.
If a row is squeezed-out for $x$-bit, we delay the input of these rows for $x$ clocks, which implemented by Fig.~\ref{fig:architecture} \hquan{D} and will be discussed in Section~\ref{sec:modules}.
% If the squeeze-out degree $x$ of the rows of bit matrix \textgreater$\ 0$, we delay the input of these rows for $x$ clocks, which implemented by Fig.~\ref{fig:architecture} \hquan{D} and will be discussed in Section~\ref{sec:modules}.

% For example, as shown in the Fig.~\ref{fig:algorithm-framework}(2), we squeeze the first row along the bit-width with the squeeze-out degree $x=1$, which is equal to shift the weight of the first row to left once($weight/2$) (e.g., $W1$ changes from $0.875 = 11100000$ to $0.4375 = 01110000$). And the inputs of all the rows in the bit matrices are the same;  thus, we shift the input one bit to the right ($input\times2$), which acts on each bit of the weight in the first row. This can make up for the changes in squeezed weight (e.g. $I\times W1 =(I\times2)\times(W1/2)$).


Assume that the weights and inputs are both 8-bit and the row is squeezed-out by 1-bit.
%the squeeze-out degree $x = 1$. 
For example, in Fig.~\ref{fig:algorithm-framework}(2), the first row in BM$_1$ is non-empty. Starting from BM$_1$, the bit matrix's non-empty rows are placed at the same position as the latter bit matrix, and the rows of the last bit matrix are squeeze-out and drop out. % then passed to the bit matrix in turn until the squeezed rows of the last bit matrix are discarded. 
After that, the crossbar storing MSB (i.e., $2^{-1}$) can be saved, and the bit-width of weights changes from $8$- to $7$-bit. The bits represent the $2^{-1}$ stored in the bit matrix represent $2^{-2}$, which means the part of weight is shrunk by half (i.e., $W1$ changes from $0.875 = 11100000$ to $0.4375 = 01110000$). And the input of row in the bit matrices are the same; thus, we shift the input of the first row one bit to the right ($input\times2$), which acts on the first row in each bit matrices to make up for the changes in weight (e.g. $I1\times W1 =(I1\times2)\times(W1/2)$). This process equal to delay the input one cycle, which means the cycle of input changes from $8$ to $9$. As a result, the total amount of computation changes from $8\times H\times W\times 8$ to $9\times H\times W\times 7$, the computation has been reduced.
% The cycle of input changes from $8$ to $9$, which means the initial input cycle is delay and equal to multiple $2$. And the total amount of computation changes from $8\times H\times W\times 8$ to $9\times H\times W\times 7$, the total amount of computation has even been reduced.



==> background_original.tex <==
\begin{figure*}[thbp]
% \setlength{\abovecaptionskip}{3pt}
\centering
\includegraphics[width=1\linewidth]{image/distribution-vs-int8.pdf}
% \includegraphics[scale=0.3]{image/distribution-new-crop.pdf}
\caption{Comparison of the INT8 and logarithmic quantization indicated by the histogram of bit-level sparsity of different weight bits in convolution layer of various quantized DNNs on ImageNet dataset~\cite{deng2009imagenet}. Thanks to the weights encoded in binary representation (i.e., $w\approx  \pm \sum_{i=1}^{8} b_i\cdot 2^{-i},~b_i\in\{0,1\}$) and logarithmic quantization and mapping scheme, a significant portion of crossbar that corresponds to certain bits are highly sparse, which inspires us to exploit this sparsity to improve crossbar utilization.}
\label{fig:distribution}
\end{figure*}
\subsection{Quantization}
\begin{figure}[bph]
\setlength{\abovecaptionskip}{3pt}
\centering
\includegraphics[width=0.9\linewidth]{image/ReRAM-overview-m1.pdf}
\caption{In-situ computation based on the ReRAM crossbar.}
\label{fig:reram}
\end{figure}
Quantization is one of the mainstream compression methods to reduce the complexity of DNN models, which maps the weight values distributed from the infinite space of real numbers to the finite space of discrete numbers with less bit-width. Especially, quantization is not just a compression step, it is a must-have step for allowing ReRAM crossbar to accelerate the DNN inference.
% \noindent\textbf{Weight Quantization}attempts to reduce the bit-width of operands in the calculation and leverage the redundancy in the bit-widths of weights, which can shrink the model size for memory saving and simplify the operations for compute acceleration.

% Many of the prior works~\cite{leng2018extremely,esser2020LSQ} pursue quantizing the model with extremely low bit-width. They have to adopt an iterative quantization and retraining/fine-tuning method to learn the network characteristic from the degree of accuracy degradation during quantization steps. 
INT8 quantization is a method that is widely used in weight compression. It converts the weight value into an integer to participate in the calculation, and the final output is multiplied by the sacle coefficient to restore. The logarithmic quantization~\cite{li2019additive,fangxin2020ausn} stores the exponent in the bit-width, which is a good candidate for quantization to facilitate hardware implementation. These methods leverage the superposition of multiple exponents to quantize the weights (in equation~\ref{con:equ0}) with negligible accuracy loss and the binary encodings of the quantized weights naturally match the SLC-based crossbar:
\begin{equation}
\setlength\abovedisplayskip{3pt}%shrink space
\setlength\belowdisplayskip{3pt}
Q(weight) =  \gamma\times(\sum_{i=0}^{n-1} 2^{p_i}), \quad p_i\in\mathbb Z
\label{con:equ0}
\end{equation}
Where $\gamma$ is a scaling coefficient to make weight into the range of $[0,1]$, $p_i$ is the exponent of power-of-two and $n$ is the number of power-of-two terms for superposition.


\subsection{Crossbar-based Vector-Matrix Multiplier}
ReRAM crossbar is emerging as a promising solution to mitigate problems such as memory wall, owing to its high memory accessing bandwidth and high density~\cite{chi2016prime,shafiee2016isaac,chou2019cascade,song2017pipelayer,nag2018newton,ankit2019puma,li2020timely,yao2020fully}. 
% ReRAM is a type of emerging non-volatile memory, which stores the information using its resistance. 
The existing researches about ReRAM-based NN accelerators use a mass of crossbar arrays and treat the ReRAM crossbar as a low-precision, low-energy and high-speed dot-product engine.
% Neural Network applications are computation- and memory- intensive, making it difficult to be deployed to embedded systems with limited resources. Therefore, there are massive accelerators based on mature digital circuits to speedup DNN computations~\cite{chen2014dadiannao,parashar2017scnn,zhang2016cambricon,song2020gpnpu,song2020drq}. ReRAM crossbar is emerging as a promising solution to mitigate problems such as memory wall, owing to its high memory accessing bandwidth and high density~\cite{chi2016prime,shafiee2016isaac,chou2019cascade,song2017pipelayer,nag2018newton,ankit2019puma,li2020timely,yao2020fully}. ReRAM is a type of emerging non-volatile memory, which stores the information using its resistance. The existing researches about neural network accelerators based on ReRAM use a mass of crossbar arrays and treat the ReRAM crossbar as a low-precision, low-energy and high-speed dot-product engine.
Digital inputs are first converted into analog voltages using digital-to-analog converters (DACs). These voltages are applied on each bit-line and the output current on each source-line collects the current of all the cells in that column according to the Kirchhoff’s law. Then, analog-to-digital converters (ADCs) convert these current into digital value to go through further calculation (as shown in Fig.~\ref{fig:reram}).


\subsection{ReRAM-based Sparse NN Accelerators} SRE~\cite{yang2019sparse} and SmartExchange (SE)~\cite{zhao2020smartexchange} are the recent ReRAM-based Sparse NN Accelerators, which improve performance by leveraging the unstructured sparsity with heavy overhead. Specifically, SRE considers the limitation of the number of rows of the crossbar for concurrent execution of MACs and designs the sparsity utilization strategy based on the ``smaller crossbars'', namely Operation Units (OUs). SmartExchange generates and utilizes the irregular sparsity in the weights to reduced energy consumption and improve the latency performance by designing a unified framework. However, such design results in significant throughput degradation, sophisticated design, a limited compression rate, and massive routing overhead.


\subsection{Motivation}
As shown in Fig.~\ref{fig:distribution}, the most significant bits of the binary codeword are very sparse since the long-tail effect in the weights of convolution layers that few weights have sizeable absolute value. Also, different quantization methods lead to different kinds of sparsity. For instance, logarithmic quantization generates more sparsity on the crossbar compared with INT8. Suppose we deploy the quantized weight on the crossbar with the conventional mapping method, which maps the bits of a quantized weight onto adjacent ReRAM-crossbar cells~\cite{shafiee2016isaac,chi2016prime,chou2019cascade,yao2020fully}, namely intra-crossbar mapping. In that case, even if quantization methods generate massive bit-level sparsity, it is difficult to exploit this sparsity (i.e., sparse cells) efficiently. 
In summary, the limitation of utilizing the sparsity in algorithm and hardware still exists in the ReRAM-based crossbar hardware, which is due to the crossbar structure tightly coupled with data. 
% As shown in Fig.~\ref{fig:comparsion-int8} (a) and (b), deploy the quantized weights by INT8 to the crossbar with conventional mapping method, resulting in the scattered distribution of sparsity on crossbar. In contrast, there is massive and regular sparsity on the crossbar quantized by logarithmic quantization.
% Even the more bit-level sparsity, however, cannot be exploited to improve the crossbar performance. \par
We believe it is the critical stumbling block for future ReRAM-based accelerators. This paper, therefore, trives to deeply decoupled it through maximally decoupling the bit-level sparsity with the crossbar architecture to release the bit-level sparsity in weights while respecting the NN accuracy and improving accelerator performance.


\begin{figure}[htbp]
\centering
\includegraphics[scale=0.14]{image/comparsion_INT8_v2.pdf}
\caption{Comparison of conventional INT8 quantization (a) and logarithmic quantization (b) for deploying model onto SLC-based crossbars.}
% \caption{Comparison of our method and conventional method for deploying the model to crossbars. (a) The conventional method leads to scattered distribution of sparsity on crossbar. (b) Our quantization generates massive and structural sparsity on the crossbar. (c) The massive sparsity is decoupled with crossbar and can be used to save crossbar resources, which benefits from the combination of our encoding and mapping.}
% \caption{Our quantization \& inter-crossbar mapping scheme vs. conventional quantization \& intra-crossbar mapping. (a) Deploy the quantized weights by INT8 to the crossbar with conventional mapping method, resulting in scattered distribution of sparsity on crossbar. (b) Due to our quantization, there is massive and regular sparsity on the crossbar, but the sparsity is tightly coupled with the crossbar, which leads to utilizing to save resources difficultly. (c) The massive sparsity is decoupled with crossbar and can be used to save crossbar resources, which benefits from the combination of our encoding and mapping.}
\label{fig:comparsion-int8}
\end{figure}
